Superselection sectors in the 3d Toric Code

We rigorously define superselection sectors in the 3d (spatial dimensions) Toric Code Model on the infinite lattice $\mathbb{Z}^3$. We begin by constructing automorphisms that correspond to infinite flux strings, a phenomenon that's only possible in open manifolds. We then classify all ground state superselection sectors containing infinite flux strings, and find a rich structure that depends on the geometry and number of strings in the configuration. In particular, for a single infinite flux string configuration to be a ground state, it must be monotonic. For configurations containing multiple infinite flux strings, we define "infinity directions" and use that to establish a necessary and sufficient condition for a state to be in a ground state superselection sector. Notably, we also find that if a state contains more than 3 infinite flux strings, then it is not in a ground state superselection sector.

==> Main/straightening.tex <==
\section{Proof of the straightening procedure}
\label{app:straight}
    First consider the case where $\dg$ is parallel to one of the principal planes, say the $x-y$ plane, and assume it is non-monotonic along the $x$ direction. The proof proceeds identically for any other choice of principal plane and axis along which the path is non-monotonic. Choose $a,b,c \in \mathbb{Z}$ such that $c = (\partial_0 \dg(n))_x = (\partial_1 \dg(m))_x$, and $a = (\partial_0 \dg(n))_y, b = (\partial_1 \dg(m))_y$. Now construct a finite path $\dg''$ such that $\dg'' (p) = \edge((c,a + p,0);\hat{y})$ for $0\le p \le b - a -1$. Here $\edge(v;\hat{r})$ is an edge starting from $v$ pointing in the $\hat{r}$ direction.\\
    
    Finally, construct a new path $\dg'$ as follows:
    \begin{align*}
        \dg'(p) &= \dg (p) &p < n\\
        \dg'(p) &= \dg''(p-n) &n\le p < n+b-a\\
        \dg' (p) &= \dg (p-(n+m + b-a -1)) &p \ge n+b-a
    \end{align*}
    $\dg'$ is path equivalent to $\dg$ and has fewer dual edges in the region where $\dg$ is non-monotonic. From proposition \ref{pro:EnergyBdy}, we see that $\omega_{\dg'}$ has a lower energy than $\omega_{\dg}$. Thus $\omega_{\dg}$ could not have been the ground-state.\\

    Now consider the case where it is non-monotonic in 2 directions, say along $x,z$. The proof is identical for a different choice of directions along which the path is non-monotonic. Define a projection ($P_{z}$) of this path into the $x-y$ plane through the following method:
    \begin{align*}
        P_{z} (\dg) :=& \dg_z &\\
        \dg_z(t) =& \dg(t) & \dg(t) \in \edge^{r,\pm}, r\in\{x,y\} \\
        =& \emptyset & \dg(t) \in \edge^{z,\pm}
    \end{align*}
    This will give us a possibly finite path lying in the $x-y$ plane. This way we obtain a path that is now only non-monotonic in $x$. We can now apply the previous analysis to show that $\dg_z$ is not the ground-state, by obtaining a path $\dg'_z$ which has a lower energy. Then we can lift the path back up into the 3d region and get that indeed $\omega_\dg$ could not have been the ground-state. Let us define a lift function $\mathcal{L}: (\dg, \dg) \rightarrow \dg$ that takes as input the paths $\dg, \dg'_z$ and outputs the lifted path $\dg'$:
    \begin{align*}
        \mathcal{L}(\dg(t), \dg'_z(t))&:= \dg'_z (t) & \dg'_z(t) \neq \emptyset\\
        &= \dg(t) & \dg'_z(t) = \emptyset
    \end{align*}
    
    
    We have now obtained a new curve $\dg'$ which is monotonic in $x,y$. We can eliminate the non-monotonicity in the $z$ direction by repeating this procedure and projecting the path into the $y-z$ plane. Figure \ref{fig:straightening} shows how to straighten a curve that is non-monotonic in 2 directions.\\

    In the case that the path is non-monotonic in all 3 directions, we can always choose a smaller region where the path is monotonic in at least one of the principal directions. This concludes the proof.
